Nonlinear Temperature Sensitivity of Residential Electricity Demand: Evidence from a Distributional Regression Approach

We estimate the temperature sensitivity of residential electricity demand during extreme temperature events using the distribution-to-scalar regression model. Rather than relying on simple averages or individual quantile statistics of raw temperature data, we construct distributional summaries, such as probability density, hazard rate, and quantile functions, to retain a more comprehensive representation of temperature variation. This approach not only utilizes richer information from the underlying temperature distribution but also enables the examination of extreme temperature effects that conventional models fail to capture. Additionally, recognizing that distribution functions are typically estimated from limited discrete observations and may be subject to measurement errors, our econometric framework explicitly addresses this issue. Empirical findings from the hazard-to-demand model indicate that residential electricity demand exhibits a stronger nonlinear response to cold waves than to heat waves, while heat wave shocks demonstrate a more pronounced incremental effect. Moreover, the temperature quantile-to-demand model produces largely insignificant demand response estimates, attributed to the offsetting influence of two counteracting forces.

==> FRKETQ_P3/01_FRKET_Intro.tex <==
\noindent Accurately estimating electricity demand during extreme weather events is vital for ensuring energy security and enhancing grid reliability. For energy practitioners and policymakers, precise demand estimation is crucial for managing supply and demand, preventing power outages, and ensuring that the energy infrastructure can withstand increased loads during such critical periods. As climate change leads to more frequent and severe weather conditions, precise demand estimation becomes a key priority for sustainable energy management.

% (Research Question, KS will do this by August)
\indent The unexpected spikes in electricity demand during extreme temperature events present unique challenges that require advanced econometric modeling to ensure grid reliability. It is known that residential electricity demand is highly sensitive to temperature changes, and extreme weather can lead to nonlinear increases in demand, placing significant stress on grid infrastructure. Electricity demand would be substantially underestimated without accurately capturing these nonlinearities, risking grid stability. Therefore, modeling the nonlinear relationship between temperature and electricity demand is essential to inform effective energy management strategies and secure the grid's resilience against future weather extremes.

\indent The key challenge in estimating the nonlinear relationship between electricity demand and temperature lies in the assumption that nonparametrically estimated temperature densities are treated as true densities. This assumption can introduce bias into demand response estimates since errors from the estimation process may distort the results. Furthermore, generating a representative temperature density using hourly regional data adds further estimation errors, which can lead to biased and inconsistent demand response estimates. These errors are particularly problematic during extreme temperature events, compromising the reliability of forecasts critical for energy security and grid stability.

\indent Building on the foundational work of \cite{engle1986semiparametric}, a substantial body of literature has applied the cointegration framework for analyzing electricity demand, with noticeable contributions from \cite{engle1989merging}, \cite{silk1997short}, \cite{beenstock1999demand}, \cite{chang2014time}, \cite{chang2016disentangling}, and \cite{chang2021forecasting}, among others. Subsequently, the literature has focused on incorporating nonlinear temperature variables, such as Heating Degree Days (HDD) and Cooling Degree Days (CDD), or employing nonlinear econometric methods to evaluate the impact of temperature fluctuations on electricity demand, including \cite{sailor1997sensitivity}, \cite{henley1997non}, \cite{henley1998residential}, \cite{valor2001daily}, \cite{pardo2002temperature}, and \cite{apadula2012relationships}. In particular, smooth transition, panel threshold, and switching regression models have been employed to capture nonlinear demand responses (\citealp{moral2005modelling}; \citealp{bessec2008non}). More recently, density-based functional approaches have emerged to analyze these effects across sectors, providing deeper insights into the nonlinearity between temperature and electricity demand (\citealp{chang2016new}; \citealp{miller2022modeling}).

\indent The nonlinear relationship between electricity demand and temperature has been further explored through various advanced methodologies. For instance, \cite{teixeira2017} integrated linear regression with artificial neural networks to capture diverse consumption patterns, while \cite{caro2020} and \cite{sharma2020} utilized periodically correlated models and synergy of recurrent neural networks with fuzzy logic, respectively, to enhance load forecasting accuracy. Meanwhile, \cite{sigauke2013extreme} applied tail-quantile estimation to analyze extreme daily increases in peak electricity demand, highlighting the critical role of temperature-driven demand fluctuations. Lastly, \cite{sultana2022} refined short-term demand forecasts using machine learning, focusing on managing temperature-induced variability.

\indent Compared to the existing literature, we introduce a functional econometric approach that effectively captures the nonlinearity of residential electricity demand response, even in the presence of measurement errors—a dimension that has not been thoroughly addressed in the existing literature. By addressing the complexities introduced by the measurement errors, our approach provides a more robust estimation, setting it apart from traditional techniques that may overlook these critical factors. Furthermore, our approach differs significantly from existing studies by focusing on the nonlinear demand response of residential electricity to changes in temperature density, rather than just temperature levels. This allows for a more comprehensive analysis, capturing the broader distributional effects of temperature fluctuations, particularly during extreme weather events. By examining shifts in the entire temperature distribution, we provide deeper insights into how extreme temperatures impact electricity demand.

\indent Instead of viewing density and quantile functions as competing methods, we consider them complementary strategies, each providing unique insights to form a comprehensive analytical framework. The density-based approach offers direct interpretability within a compositional data framework, allowing for clear analysis of temperature's impact on electricity demand across the entire distribution. On the other hand, quantile functions address heterogeneous support more effectively and excel in estimating the cumulative effects of temperature at highest or lowest quantiles. Notably, these issues have not been adequately addressed in the existing literature. In this paper, we apply the Centered-Log-Ratio (CLR) transformation for density-valued functional data and mean centering for quantile-valued functional data. These transformations enable us to handle the distinct characteristics of each functional data, providing a more robust analysis.

\indent The remainder of this paper is structured as follows. Section \ref{sec_method} details the econometric methodology employed to estimate the nonlinear response of residential electricity demand in the presence of measurement errors. Section \ref{Sec_Data} discusses the residential electricity demand and local temperature data from the Republic of Korea. Given two extreme weather events, Section \ref{Sec_Empirics} presents empirical results illustrating the nonlinear sensitivity of temperature density and quantile functions. Finally, Section \ref{Sec_conclude} provides concluding remarks, with econometric proofs included in the Appendix.




==> FRKETQ_P3/02_FRKET_Econometrics.tex <==

\subsection{Distributional predictors of temperature and measurement errors} \label{sec_method_1}
We let $y_t$ be the electricity demand, a practical measurement of which is detailed in Section \ref{Sec_Data}, and $X_t^\circ$ be a functional object that summarizes the distributional properties of temperature. There may be various choices for $X_t^\circ$, but we in this paper focus on two choices,  (i) the CLR transformation and (ii) quantile function corresponding to the probablity density function, denoted $p_t$, of temperature. The former seems to be a standard choice in the literature, and the latter has it own merit, compared to the former, to our empirical application.  

If the density $p_t$ of temperature is supported on $[a,b]$, then the CLR transformation $X_t^\circ$  of $p_t$ is defined as follows:
\begin{equation}\label{eqclr}
	X_t^\circ(r) = \log p_t(r) - \int_{a}^b \log p_t (s) ds, \quad r\in [a,b] 
\end{equation}
%As discussed in the recent literature, it is not advisable to consider the original density function of temperatures, say $p_t$, as the predictor $X_t^\circ$. This is because that the nonlinear restrictions (i) $p_t(r)\geq 0$ for all $r\in [a,b]$ and (ii) $\int_{a}^b p_t(r) dr=1$, which are essentially required for $p_t$ to be a proper density, prevent us from using the existing well-developed statistical theory developed in a Hilbert space setting (see e.g., \citealp{petersen2016,Hron2016330,SEO2019}). As a way to circumvent this issue, we consider the following CLR transformation of $p_t$, which were earlier proposed in the literature (\citealp{Egozcue2006}) :
Under some mathematical conditions on the underlying probability density $p_t$, the transformation from $p_t$ to its CLR transformation not only embeds the probability densities on $[a,b]$ into a linear subspace of the $L^2[0,1]$ Hilbert space but also is invertible. Thus, the CLR transfomration of $p_t$ have been considered a standard choice in the model involving distributional functional data (see e.g., \citealp{kokoszka2019forecasting,SEO2019,seong2021functional})

We also let $X_t^\circ$ be the quantile function corresponding to $p_t$, i.e.,  
\begin{equation}\label{eqqf}
	X_t^\circ(r)  = \inf \{x \in [a,b]:\int_{a}^{x} p_t(s) ds \leq r\},  \quad r\in [0,1].   
\end{equation}
It is well known that, for the CLR transformation to be an invertible transformation of a set of probability densities, $p_t$ needs to be supported on a common compact interval $[a,b]$ for every $t$ (see e.g., \citealp{Egozcue2006,Boogaart2014}). This requires us to estimate all the temperature densities on a common interval. On the other hand, the quantile functions do not require such a restriction, and the support of the function can vary over time. 

In practice, $p_t$ cannot be directly observed, and thus $X_t^\circ$ is not observable. For empirical analysis, it needs to be constructed from the raw temperature data; specifically, we may replace $p_t$ or $\log p_t$ with relevant nonparametric estimate in \eqref{eqclr} (as in \citealp{SEO2019}) or replace population quantiles with sample quantiles in \eqref{eqqf}. However, this replacement necessarily introduces estimation/smoothing errors, and may lead inconsistent estimation of the model. Subsequently, we discuss econometric methods for studying the distributional impact of temperature on electricity demand that are robust to the presence of these estimation/smoothing errors contained in the distributional predictor. 

%\noindent In empirical studies involving density- or quantile-valued functional data, two challenges arise: (i) the nonlinear constraints make simple functional data analysis inadequate for properly defining these functions within a Hilbert space, and (ii) the true density or quantile function of an economic or climate variable is unobservable, requiring nonparametric density or quantile estimates as proxies. 

%\indent To address the first challenge, researchers often apply invertible transformations such as the CLR transformation introduced by \cite{Egozcue2006} to the estimated density functions. As such, we first apply the CLR transformation to the time series of the temperature density function.\footnote{A small value of 0.001 is added to the entire temperature density function to conduct the CLR transformation over the common support range of $[-20,40]$.} We then incorporate the hypothetically generated functional shocks based on the CLR-transformed and temporally demeaned functional data. These CLR-transformed temperature density functions, along with the functional shocks, are represented in the function space using orthonormal Fourier basis vectors.

%\indent Unlike density functions, which exploit the CLR transformation to define linear operators for Hilbert space analysis, quantile functions lack an appropriate invertible transformation, making Hilbert space analysis more challenging. Quantile functions map quantiles to temperature values without the constant sum constraint inherent in density functions. This limitation complicates quantile function analysis within the Hilbert space. Acknowledging this limitation, we simply apply a mean centering operation to represent the quantile function in the function space using Fourier basis functions. 

%\indent Regarding the second challenge, researchers typically replace unobservable true density or quantile function with nonparametric density or quantile estimates, and these estimates would be susceptible to measurement errors. As discussed earlier, such measurement errors—stemming from data quality issues or limitations in the estimation process itself—can lead to inconsistent estimates, introducing bias into the analysis of nonlinear responses, particularly regarding temperature's impact on electricity demand. In this light, addressing measurement error is critical for accurately uncovering the true nature of nonlinear demand response, underscoring the need for more robust methodologies.



\subsection{Econometric model and estimator} \label{Sec_Model}
For the subsequent discussion, it will be convenient to introduce some essential notation. We let $\mathcal H$ be the Hilbert space of square-integrable functions defined on $[a,b]$ with inner product $\langle g,h \rangle = \int_{a}^b g(s)h(s)ds$ for and norm $\|g\|=\sqrt{\langle g,g \rangle}$, where $g,h \in \mathcal H$; $\mathcal H$ is a commonly considered Hilbert space in the literature on functional data analysis. The distributional predictor $X_t^\circ$ and its measurement $X_t$,  which are introduced in \eqref{sec_method_1}, are understood as random elements in $\mathcal H$. Essential concepts on $\mathcal H$ and notation, which we subsequently consider, are reviewed in Section \ref{sec_app_prelim}. 

To study temperature sensitivity of electricity demand, we consider the following model: 
\begin{equation} \label{eqreg1}
	y_t = \mu +  f (X_t^{\circ}) + \varepsilon_t,
\end{equation}
where $f:\mathcal H\mapsto \mathbb{R}$ is a linear map, connecting $y_t$ and $X_t^{\circ}$,\footnote{The linear map $f$ can be equivalently expressed as an integral transformation associated with a kernel function $\mathrm k_f$, as follows: $	f(X_t^{\circ}) = \int_{a}^b \mathcal \mathrm k_f (r) X_t^{\circ}(r)dr$. Obviously, estimation $\mathrm{k}_f$ is identical to estimation of $f$. However, we in this paper, focus on $f$.}  and $\mathbb{E}[ \varepsilon_t] = 0$.
\eqref{eqreg1} pertains to the function-to-scalar regression (FSR) model, which is extensively discussed in the literature.  As discussed in Section \ref{sec_method_1}, in practice, $X_t^\circ$ is not directly observed and has to be estimated or smoothed from discrete samples $\{p_t^{\circ} (s_i)\}_{i=1}^{N_t}$ of $p_t$, and practitioners often have no choice but to replace $X_t^{\circ}$ with its feasible estimate $X_t$. As earlier pointed out by \citet[Sections 2 and 5.3]{seong2021functional}, this is a common source of endogeneity in the regression model involving functional data, and ignoring such errors may be detrimental to the use of standard estimators of $f$, requiring the exogeneity of the predictor, developed in the literature. 

To illustrate this issue with a concrete example, we assume that $X_t = X_t^{\circ} + e_t$, where $e_t$ measures the additive departure of $X_t$ from $X_t^{\circ}$ and is assumed to satisfy $\mathbb{E}[e_t]=0$. Then, from \eqref{eqreg1},  we find that the following relationship holds:
\begin{equation} \label{eqreg2}
	y_t = \mu+  f (X_t) + u_t, \quad u_t =  f(e_t) + \varepsilon_t,
\end{equation}
where $\mathbb{E}[u_t] = 0$ holds. In the above, $X_t$ and $u_t$ are generally correlated, i.e., $\mathbb{E}[X_t\otimes u_t] \neq 0$), where $\otimes$ denotes the tensor product (see Section \ref{sec_app_prelim} of Appendix).\footnote{Specifically, for any $g,h$ taking values in $\mathcal H$, $	g \otimes h (x) = \langle g,x \rangle h = (\int_{a}^{b} g(s)x(r)dr)h$ for any $x\in \mathcal H$.} 
As is well known in the literature (see e.g., \citealp{seong2021functional}, Sections 1--2), this endogeneity makes the standard estimators, developed under the exogeneity condition $\mathbb{E}[X_t\otimes u_t]=0$, inconsistent and inferential methods associated with those estimators invalid. 

To estimate $f$ from \eqref{eqreg2} and implement valid statistical inference, we in this paper adapt the functional IV estimator developed for function-to-function regression (FFR) model to our context. To this end, we let $Z_t$ be the functional Instrumental Variable (IV) satisfying the following conditions: 
\begin{align}\label{eqreg3}
	C_{XZ}:=\mathbb{E}[(X_t-\mathbb{E}[X_t])\otimes (Z_t-\mathbb{E}[Z_t])]\neq 0, \quad 
	C_{Zu}:=\mathbb{E}[Z_t\otimes u_t]=0. %\, \text{ or equivalently }\,   C_{Zy}:=\mathbb{E}[Z_t\otimes y_t] = f C_{XZ}^\ast, 
\end{align}
The above consists of only the minimal requirements for the IV $Z_t$. More conditions for the consistency and (local) asymptotic normality of our estimator will be detailed in Section \ref{sec_app_est} of  Appendix.
ssuming that the measurement errors are not serially correlated and $X_{t}$ exhibits a time series dependence,  in our empirical analysis we will let $Z_t$ be a lagged distributional predictor as in \citet[Section 5.3]{seong2021functional}. To obtain our proposed estimator, we need to compute the sample covariance operators $\widehat{C}_{XZ}$ and its adjoint $\widehat{C}_{XZ}^\ast$ as follows:
\begin{equation}\label{eqcxz}
	\widehat{C}_{XZ} = \frac{1}{T}\sum_{t=1}^{T} (X_t-\bar{X}_T) \otimes (Z_t-\bar{Z}_T), \quad \widehat{C}_{XZ}^\ast = \frac{1}{T}\sum_{t=1}^{T} (Z_t-\bar{Z}_T) \otimes (X_t-\bar{X}_T), 
	%\widehat{C}_{Zy} = \frac{1}{T}\sum_{t=1}^{T} Z_t \otimes y_t, \quad
	% \quad %\widehat{C}_{Zu} = \frac{1}{T}\sum_{t=1}^{T} Z_t \otimes u_t, 
	%\widehat{\Gamma}_{yX} =\widehat{C}_{Zy} \widehat{C}_{XZ}, \quad   \widehat{\Gamma}_{X} = \widehat{C}_{XZ}^\ast \widehat{C}_{XZ},
\end{equation}
where $\bar{X}_T=T^{-1}\sum_{t=1}^T X_t$ and $\bar{Z}_T=T^{-1}\sum_{t=1}^T Z_t$. $\widehat{C}_{XZ}$ and $\widehat{C}_{XZ}^\ast$ are, respectively, the sample counterparts of $C_{XZ}$ and $C_{XZ}^\ast (:=\mathbb{E}[(Z_t-\mathbb{E}[Z_t])\otimes (X_t-\mathbb{E}[X_t])])$.  As is well known in the literature, $\widehat{C}_{XZ}^\ast \widehat{C}_{XZ}$ allows the eigendecomposition with respect to its eigenvalues $\{\hat{\lambda}_j^2\}_{j\geq 1}$ and eigenvectors $\{\hat{g}_j\}_{j\geq 1}$, i.e., 
\begin{equation}
	\widehat{C}_{XZ}^\ast \widehat{C}_{XZ} = \sum_{j=1}^\infty \hat{\lambda}_j^2 \hat{g}_j \otimes \hat{g}_j.
\end{equation}
The eigenelements can be computed using the standard functional principal component analysis (FPCA) as in \cite{seong2021functional}. 
Then our proposed estimator $\hat{f}$, which is a map from $\mathcal H$ to $\mathbb{R}$, is defined as follows: for any $x \in \mathcal H$,
\begin{align} \label{eqest}
	\hat{f}(x) = T^{-1}\sum_{t=1}^T \sum_{j=1}^{\KK} \hat{\lambda}_j^{-2} \langle \hat{g}_j, x \rangle \langle \widehat{C}_{XZ}\hat{g}_j,Z_t-\bar{Z}_T \rangle  (y_t-\bar{y}_T),
\end{align}
where $\bar{y}_T=T^{-1}\sum_{t=1}^T y_t$ and $\KK$ is sufficiently smaller than $T$; a more detailed and technical requirement on the choice of $\KK$ will be postponed to Section \ref{sec_app_est} of Appendix. If $\KK$ is appropriately determined, it is straightforward to compute the estimator using  $\widehat{C}_{XZ}$ and the sample eigenelements $\{\hat{\lambda}_j^2,\hat{g}_j\}$. The above estimator is in fact a sample analogue estimator based on the population equation $C_{Zy}C_{XZ}= f C_{XZ}^\ast C_{XZ}$, which holds when $Z_t$ satisfies \eqref{eqreg3} (see Section \ref{sec_app_est} of Appendix for more detailed discussion.). From this equation, the estimator \eqref{eqest} is obtained by (i) replacing the population operators $C_{Zy}$ and $C_{XZ}$ with their sample counterparts $\widehat{C}_{XZ}^\ast \widehat{C}_{XZ}$ and then (ii) employing a regularized inverse of $\widehat{C}_{XZ}^\ast \widehat{C}_{XZ}$, which is necessary to compute the estimator.

Adapting the theoretical results developed for FFR model by \cite{seong2021functional}, we establish the consistency of $\hat{f}$ under appropriate assumptions as follows:
\begin{proposition}\label{prop1}
	Under Assumption \ref{assum1} given in Section \ref{sec_app_est}, $\hat{f}$ is a consistent estimator of $f$. 
\end{proposition}
Proposition \ref{prop1} is intentionally presented without any mathematical details; a more rigorous version is provided in the Appendix (see Proposition \ref{prop1a}). The consistency stated in Proposition \ref{prop1} implies that for every $x \in \mathcal{H}$, $\hat{f}(x)$ converges in probability to $f(x)$. 

It is often of interest for practitioners to see the effect $f(\zeta)$ on $y_t$ of a specified distributional perturbation $\zeta$ given to $X_t^\circ$; \commWK{specifically, in our empirical analysis, $\zeta$ will be set to extreme temperature events, called heat wave and cold wave, and we are interested in the effect of these events on $y_t$.} The consistency result given by Proposition \ref{prop1} implies that this effect can be estimated by $\hat{f}(\zeta)$. Beyond the consistent estimation, the following results, which can be used for statistical inference on $f(\zeta)$, can be established under some appropriate conditions (see Proposition \ref{prop2} in the Appendix):  
\begin{equation}\label{eqlocal}
	\sqrt{\frac{T}{\hat{\sigma}^2_u \widehat{\theta}_{\KK}(\zeta)}}(\hat{f}(\zeta)-f(\zeta)) \to_d N(0,1),
\end{equation}
where   $\hat{\sigma}^2_u$ is the sample variance of $u_t$, which is computed from the residuals $\hat{u_t} = y_t-\hat{f}(X_t)$, and
\begin{equation} \label{eqtheta}
	\widehat{\theta}_{\KK}(\zeta) %= \langle \hat{\zeta}, \widehat{C}_{ZZ} \hat{\zeta} \rangle,  \quad \text{with} \quad  \hat{\zeta} = \sum_{j=1}^{\KK} \hat{\lambda}_j^{-2} \langle \hat{g}_j,\zeta \rangle \widehat{C}_{XZ}\hat{g}_j. 
	=\frac{1}{T} \sum_{t=1}^T \left(\sum_{j=1}^{\KK} \hat{\lambda}_j^{-2} \langle \hat{g}_j, \zeta\rangle \langle \widehat{C}_{XZ}\hat{g}_j, Z_t-\bar{Z}_T\rangle\right)^2.
\end{equation}
This result may be understood as the local asymptotic normality of the functional IV estimator, which was earlier obtained by \cite{seong2021functional} in the FFR model.


==> FRKETQ_P3/03_FRKET_Data.tex <==
\subsection{Raw data and temperature densities} \label{Sec_Data_1}

\noindent To investigate nonlinear temperature sensitivity while accounting for potential measurement errors, we analyze an extensive dataset that includes residential electricity demand (unit: GWh) and local temperature (unit: degrees Celsius) readings from the Republic of Korea, covering the period from January 1999 to December 2023 (300 monthly observations). The residential electricity demand data are provided by the Korea Electric Power Corporation (KEPCO), the state-owned utility company responsible for electricity sales across the country. Given the inherent variability in the number of days within each month, we have normalized the raw monthly electricity demand by dividing it by the number of effective days per month. This adjustment yields a metric referred to as the electricity demand per effective day, as outlined in \cite{chang2014time}, which underscores the importance of accounting for temporal differences in energy demand analysis.

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.45\textwidth, width=0.8\textwidth]{FRKETQ_P3/Y_Graph.png}
\caption{Natural log of residential electricity demand per effective day and its 12-month moving average (top), and their deviation process (down) from January 1999 to December 2023.}
\label{Fig:Y_Graphs}
\end{center}
\end{figure}

\indent \cite{chang2016new} found no empirical evidence suggesting that non-climate variables significantly influence the demand response to temperature in the residential sector. Building on this finding, and to isolate the short-run fluctuations in residential electricity demand, we calculate the deviation from the natural logarithm of a 12-month moving average of electricity demand per effective day, which are illustrated in Figure \ref{Fig:Y_Graphs}. This deviation serves as a proxy for the short-run component of electricity demand, allowing us to focus on the short-run effects of temperature changes while filtering out long-run effects of income and electricity price. By employing this detrending approach, we ensure that our analysis effectively captures the nonlinear responses of residential electricity demand to temperature fluctuations, independent of other non-climate factors.

%(heterogeneous support problem with density generation) 
\indent To model the seasonality, we retrieve the hourly temperature data from the KMA National Climate Data Center.\footnote{Downloaded from https://data.kma.go.kr/cmmn/main.do on July 1, 2024.} We then construct the monthly temperature density function over the common support, $[-20,40]$ using hourly temperature observations from the five largest cities—Seoul, Daejeon, Daegu, Gwangju, and Busan-covering the territory of the Republic of Korea.\footnote{Instead of estimating the range of the common support, we adopt the common support of $[-20,40]$ with grid difference, $0.1$, as established in the literature (\citealp{chang2014time}; \citealp{chang2016new}).} To represent the temperature density function of the Republic of Korea, we calculate the weighted average of the estimated time series for these five density functions, assigning weights based on the annual proportion of electricity sales in each of the five regions (Seoul Metropolitan Area [Seoul, Incheon, Gyeonggi], Daejeon, Daegu, Gwangju, and Busan).\footnote{The combined annual electricity consumption of the five regions accounts for approximately 55.3\% of the national total on average during the period from 1999 to 2021. Due to data availability constraints, the proportions for the years 2022 and 2023 have been substituted with the values from 2021.}\footnote{The annual regional consumption data was obtained from the Korea Energy Statistics Information System (KESIS) and can be accessed at \url{https://www.kesis.net/sub/subChart.jsp?report_id=33150&reportType=0} (data downloaded on July 1, 2024).} 

\indent Figure \ref{Fig:Quantile_descrip} illustrates the time series of a temperature density function, estimated using the normal kernel and plug-in bandwidth, and the dynamics of its descriptive statistics. Note that the generated monthly temperature density functions exhibit significant heterogeneity, particularly between summer and winter. The time-series analysis of monthly temperature distributions in the Republic of Korea from 1999 to 2023 reveals stable seasonal cycles in the mean temperature, reflecting consistent annual patterns. However, the standard deviation indicates increasing variability, particularly post-2010, suggesting a growing spread in temperature values around the mean. The skewness exhibits seasonal fluctuations, with positive skewness during warmer months indicating a higher frequency of extreme high temperatures, and negative skewness during colder months reflecting an increase in extreme low temperatures. However, this skewness does not show a clear trend of increasing asymmetry over time but rather indicates a recurring seasonal pattern. The kurtosis remains relatively stable but experiences significant spikes, particularly after 2010. These spikes suggest periods with more frequent and intense extreme temperature events. Thus, while the skewness reflects consistent seasonal variability, the spikes in kurtosis indicate a rise in temperature extremes, likely influenced by climate change. 

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.35\textwidth, width=0.4\textwidth]{FRKETQ_P3/density_desc0.png}
\includegraphics[height=0.35\textwidth, width=0.55\textwidth]{FRKETQ_P3/density_desc.png}
\caption{Kernel density estimates of the temperature distribution in the Republic of Korea (left) and the dynamics of its descriptive statistics (right). The red lines indicate August 2017 and August 2018, while the blue lines represent January 2020 and January 2021.}
\label{Fig:Quantile_descrip}
\end{center}
\end{figure}

% \indent  This non-homogeneous support presents challenges for the functional econometric methodologies, potentially rendering them inappropriate for this analysis. To address this issue, we apply the Lorenz Curve transformation combined with the quantile function, as suggested by \cite{bongiorno2019describing}, to mitigate the problem of non-homogeneous support throughout the sample period. Based on the common support range of $[-20, 40]$, more specifically, we extend the estimated quantile function by setting the 0$^\textrm{th}$ and 100$^\textrm{th}$ percentiles to the minimum and maximum values of the generated quantile functions, respectively. This approach allows the entire quantile function over the common support to capture the seasonality throughout the sample period.

% (Lorenz curve implication with L''(p) transformation) 
%\indent We generate the Lorenz curve using the formula $\hat{L}(p) = \frac{1}{\bar{X}} \int_0^p \hat{Q}(r) , dr$, where $\hat{Q}(r)$ represents the empirical quantile function at the $r$-th quantile, and $\bar{X}$ is the empirical mean of the quantile function. Next, we derive the second derivative of the Lorenz curve, $L(p)$, using the formula $L''(p) = \frac{1}{\bar{X}} f\{Q(p)\}$, where $f\{Q(p)\}$ is the density-quantile function, as presented in equation (4) of \cite{bongiorno2019describing}. Subsequently, the negative Centered-Log-Ratio (CLR) transformation is applied to the empirical $L''(p)$ to ensure it is defined within the Hilbert Space. Note that these transformation processes effectively result in the positive CLR transformation of the density function, although two different approaches would produce different results due to extended grid number and kernel estimation techniques (Do this more...).  



\subsection{Construction of the distributional predictors}
As discussed in Section \ref{sec_method_1}, distributional predictors in practice need to be estimated in advance from the raw data. For the CLR transformations, we use the estimated densities, denoted as $\hat{p}_t$, obtained in Section \ref{Sec_Data_1} (see Figure \ref{Fig:Quantile_descrip}), and construct $X_t$ as follows:\begin{equation}\label{eqclr2} X_t(r) = \log \hat{p}_t(r) - \int_{-20}^{40} \log \hat{p}_t (s) ds.\footnote{As is common in the literature (see e.g., Section 5.2, \citealp{seoshang22}), a small value of $10^{-3}$ is added to the entire temperature density function $\hat{p}_t$ to implement the log transformation over the common support range of $[-20,40]$.}  \end{equation} On the other hand, when $X_t^\circ$ is the quantile function corresponding to $p_t$, we directly estimate it from the raw temperature data by replacing population quantiles with sample quantiles.

%\indent To address the first challenge, researchers often apply invertible transformations such as the CLR transformation introduced by \cite{Egozcue2006} to the estimated density functions. As such, we first apply the CLR transformation to the time series of the temperature density function.\footnote{A small value of 0.001 is added to the entire temperature density function to conduct the CLR transformation over the common support range of $[-20,40]$.} We then incorporate the hypothetically generated functional shocks based on the CLR-transformed and temporally demeaned functional data. These CLR-transformed temperature density functions, along with the functional shocks, are represented in the function space using orthonormal Fourier basis vectors.

%\indent Unlike density functions, which exploit the CLR transformation to define linear operators for Hilbert space analysis, quantile functions lack an appropriate invertible transformation, making Hilbert space analysis more challenging. Quantile functions map quantiles to temperature values without the constant sum constraint inherent in density functions. This limitation complicates quantile function analysis within the Hilbert space. Acknowledging this limitation, we simply apply a mean centering operation to represent the quantile function in the function space using Fourier basis functions. 

%\indent Regarding the second challenge, researchers typically replace unobservable true density or quantile function with nonparametric density or quantile estimates, and these estimates would be susceptible to measurement errors. As discussed earlier, such measurement errors—stemming from data quality issues or limitations in the estimation process itself—can lead to inconsistent estimates, introducing bias into the analysis of nonlinear responses, particularly regarding temperature's impact on electricity demand. In this light, addressing measurement error is critical for accurately uncovering the true nature of nonlinear demand response, underscoring the need for more robust methodologies.


==> FRKETQ_P3/04_FRKET_Empirics_v5.tex <==
% weakness of Chang et al. (2016) approach) no clr transformation \& measurement error:  Points: Nonlinear temperature sensitivity with functional approach, CLR transformation for Hilbert space, measurement error
% errors originating from temperature measurement sites can complicate the analysis, potentially skewing density estimation and, by extension, the overall results. 

\indent Throughout this paper, we set $K$ in equation \eqref{eqest} to 3.\footnote{Following the results given in Section \ref{sec_app_est} of Appendix and Remark \ref{rem1}, we set $\KK=1+\max_{j\geq 1}\{\tilde{\lambda}_j^2 \geq \alpha\}$ for $\alpha = 0.1 \times T^{-0.3}$, where $\tilde{\lambda}_j^2=\lambda_j^2/\sum_{j=1}^\infty \hat{\lambda}_j^2$ and this is to obtain a choice of $\KK$ which is independent of the scale of $X_t$ and $Z_t$; see S5 of \cite{seong2021functional}.} \commWK{Noting that the measurement errors are caused by smoothing $X_t$ from its discrete realizations, we assume that the measurement errors are serially uncorrelated, and let $X_{t-\kappa}$ be the IV for our empirical analysis; similar approaches were earlier adopted in the numerical studies given by \cite{seong2021functional,Chen_et_al_2020}. Given that our approach relies on the autocovariance structure of the distributional predictor, it is essential to carefully select the value of $\kappa$.} A larger $\kappa$ value might lead to the loss of crucial information, particularly in capturing the temporal dynamics of the functional data. Therefore, we have chosen to set $\kappa$ to 1. This selection enables us to account for potential errors in density/quantile estimation process or data quality while minimizing the risk of information loss, thus enhancing the robustness and reliability of our analysis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Functional Shocks for Cold Wave and Heat Wave}\label{Sec_Est_Shocks}
\noindent The Republic of Korea experienced two significant extreme weather events for the sample period.\footnote{Source: \url{https://www.wunderground.com/cat6/Hottest-Day-Korean-History}, \url{https://watchers.news/2021/01/11/historic-cold-wave-and-heavy-snow-hit-south-korea/}} In August 2018, the Republic of Korea experienced one of its most intense heat waves on record, with temperatures soaring to an average of 29.2°C, the highest since record-keeping began in 1907. This extreme heat led to the residential electricity demand of 8,851.04 GWh during that month, underscoring the strain placed on the energy grid by cooling needs. Similarly, January 2021 was marked by a significant cold wave, with temperatures plunging to an average of -6.1°C, well below the seasonal norm. During this period, residential electricity demand also spiked to 7,163.28 GWh as households increased heating usage to cope with the severe cold. 

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.35\textwidth, width=0.95\textwidth]{FRKETQ_P3/Func_Shock0.png}
\caption{Kernel density estimates comparing January 2021 (solid) and January 2020 (dotted) on the left, and August 2018 (solid) and August 2017 (dotted) on the right, with the black lines representing their differences.}
\label{Fig:Func_shock2}
\end{center}
\end{figure}

\indent Figure \ref{Fig:Func_shock2} illustrates changes in the monthly temperature distributions during extreme weather events—specifically, a heat wave in August 2018 and a cold wave in January 2021. In the left panel of Figure \ref{Fig:Func_shock2}, the blue solid line represents the temperature distribution in January 2021, compared to the blue dashed line for January 2020, with the black line showing the distributional difference, capturing the effect of the cold wave. Similarly, in the right panel of Figure \ref{Fig:Func_shock2}, the red solid line represents the temperature distribution in August 2018, while the red dashed line shows the temperature distribution in August 2017, with the black line indicating the difference between these two distributions, implying the functional shock of the heat wave. 

\indent Moreover, the temperature distributions during the 2018 heat wave and the 2021 cold wave exhibit distinct shifts indicative of extreme weather conditions. The August 2018 distribution is skewed significantly to the right, reflecting a higher frequency of exceptionally high temperatures, with a pronounced right tail indicating extreme heat events. Conversely, the January 2021 distribution is heavily skewed to the left, highlighting a prevalence of unusually low temperatures, with a long left tail denoting severe cold conditions. These graphs reveal the significant shifts in temperature distributions during these extreme events, illustrating how both the heat wave and cold wave deviated sharply from typical conditions in the preceding months.% The black lines representing the differences from the previous months underscore the magnitude of these deviations, clearly illustrating the substantial impact of these climatic anomalies.

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.3\textwidth, width=0.99\textwidth]{FRKETQ_P3/Func_Shock2.png}
%\includegraphics[height=0.3\textwidth, width=0.99\textwidth]{FRKETQ_P3/Quantile_shock_Desc.png}
\caption{Selected functional shocks for cold waves (blue), shifted 50 grids to the right, and heat waves (red), shifted 50 grids to the left (left), and the mean change of the functional density shocks during the shifting process (right).}
\label{Fig:Func_shock3}
\end{center}
\end{figure}

\indent In Figure \ref{Fig:Func_shock3}, we generate functional shocks by parallelly shifting the previously mentioned shocks, in order to identify the nonlinear response of electricity demand per effective day (nonlinear demand response, in short). Specifically, the functional shock for the heat wave is shifted to the left, and the functional shock for the cold wave is shifted to the right, each across a range of one to 50 grids. By applying the CLR transformation to each shifted temperature distribution, this approach enables us to observe the functional shocks within a more moderated framework. The left panel of Figure \ref{Fig:Func_shock3} illustrates the 50-grid left-shifted heat wave shock (red dashed line) and the 50-grid right-shifted cold wave shock (blue dashed line). As expected, these shifts result in changes to the mean of the temperature distributions, as depicted in the right panel of Figure \ref{Fig:Func_shock3}. For instance, the mean temperature in August 2018 was approximately 28.54°C, compared to 26.02°C in August 2017. However, after applying a 50-grid left shift, the means of the temperature distributions were adjusted to approximately 23.55°C and 21.06°C, respectively. Thus, while the heat wave shock resulted in a mean increase of 2.49°C, shifting the temperature distributions reveals variations in the perceived impact of the heat wave shock, depending on the defined temperature level.

\indent In the left panel of Figure \ref{Fig:Func_shock3}, similarly, we observe the functional shock generated by shifting the cold wave shock (blue solid line) to the right across a range of grids. The original cold wave shock, represented by the blue solid line, shows significant deviations from the previous month, as seen in the black line in the left panel of Figure \ref{Fig:Func_shock2}. More specifically, the analysis of the cold wave shock involves comparing the temperature distributions of January 2021 and January 2020. The observed difference in mean temperatures between these two months is 3.84°C, as shown in the right panel of the figure. To preserve this difference while examining the impact of varying cold wave intensities, both temperature distributions were shifted to the right by an equal amount. Within this framework, a weak cold wave shock is defined by a shift from a temperature distribution with a mean of 7.30°C to one with a mean of 3.46°C. In contrast, a strong cold wave shock is characterized by a shift from a mean of 2.30°C to a mean of -1.53°C. These adjustments maintain the mean difference between the two distributions, while effectively illustrating how different levels of cold wave intensity can be generated and analyzed.

\indent In the cold wave scenario, as described in the right panel of Figure \ref{Fig:Quantile_descrip}, the variance for the cold wave scenario shows a significant increase from January 2020 to January 2021, reflecting a wider spread of temperatures in 2021 ($17.30 \rightarrow 51.37$). This suggests that 2021 experienced a more varied range of cold temperatures compared to the previous year. However, the skewness and kurtosis decrease for the cold wave, implying that while the temperature distribution became more dispersed, it also became more symmetrical and less peaked ($0.14 \rightarrow -0.04$ \& $2.62 \rightarrow 2.40$). This indicates that extreme cold events were less frequent in 2021 than in 2020. For the heat wave scenario, on the other hand, the variance increases much less than for the cold wave ($15.0 \rightarrow 17.11$). However, while skewness increases, kurtosis decreases, indicating that the temperature distribution in 2018 became more skewed to the right but less peaked compared to 2017 ($-0.06 \rightarrow 0.20$ \& $2.90 \rightarrow 2.50$). This suggests that extreme high-temperature events were more frequent but not as intense in 2018. Ultimately, while both cold and heat waves lead to increased variance, reflecting more extreme conditions compared to the previous year, they have different effects on the shape of the temperature distribution. The cold wave results in a more symmetrical and less extreme distribution, whereas the heat wave leads to greater asymmetry with more frequent but less intense extreme temperatures.

\bigskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Empirical Results for Density-to-Demand Model}
% (Nonlinear Temperature Sensitivity)
\begin{figure}[t]
\begin{center}
\includegraphics[height=0.5\textwidth, width=0.9\textwidth]{FRKETQ_P3/Empirical_rlt1.png}
\caption{Density-based temperature sensitivity for varying cold wave (top) and heat wave (bottom) shock intensities under $\kappa = 0$ (left) and $\kappa = 1$ (right). The black line indicates the estimation results for the orthornormal Legendre basis functions.}
\label{Fig:Empirical_rlts}
\end{center}
\end{figure}

% (economic implications) 
\indent We utilize both $80$ orthonormal Fourier basis function and $80$ orthonormal Legendre basis function to represent the distributional predictor in the function space. Figure \ref{Fig:Empirical_rlts} presents the estimation results for the density-to-demand model with Fourier (red) and Legendre (black) basis functions, incorporating the functional shocks generated by heat waves and cold waves. The dotted lines in the Figure indicate 95\% confidence intervals \commWK{for the response of $y_t$ on the specified temperature events}. The short-run estimates for $\kappa = 1$, \commWK{which is expected to effectively account for measurement errors (see e.g., \citealp{seong2021functional})}, yield particularly insightful outcomes. 

\indent The top panel illustrates the demand response to cold wave shocks (blue lines) across different temperature levels. Notably, under $\kappa=1$, which is most effective when measurement errors are \commWK{serially uncorrelated}, there is a pronounced increase in electricity demand response as temperatures drop. This suggests that colder conditions, particularly under intense cold wave shocks, significantly drive up electricity demand due to increased heating needs. The bottom panel of the figure shows the demand response to heat wave shocks (red lines), where demand response increases as temperatures increase, especially under $\kappa=1$. This reflects the heightened demand for cooling during extreme heat events. Overall, the FSR model with $\kappa=1$, where the measurement errors are modeled as \commWK{a serially uncorrelated sequence}, consistently provides the more reliable estimates, underscoring the non-linear and temperature-sensitive nature of the electricity demand response. 

\indent Note that a modest heat wave shock is defined by the distributional difference between a mean of 21.06°C and 23.55°C, with the final value of 23.55°C representing the occurrence of the heat wave shock. Similarly, the strongest heat wave shock is characterized by the difference between a mean of 26.06°C and 28.54°C, with the latter value marking the occurrence of the shock. The corresponding demand response values are 0.0591 at 23.55°C, 0.0874 at 25.95°C, and 0.0989 at 28.54°C. Given that demand is expressed in natural logarithms and that the demand response at a specific temperature reflects the relative impact of a cold or heat wave shock, the results indicate that an increase in temperature from 23.55°C to 25.95°C leads to a year-over-year monthly demand growth rate that is 2.83\% higher than the year-over-year monthly growth rate observed at 23.55°C, with demand response value rising by 0.0283 from 0.0591 to 0.0874. Furthermore, as the temperature escalates further from 25.95°C to 28.54°C, the demand growth rate increases by an additional 1.15\% compared to the year-over-year monthly growth rate at 25.95°C, with demand response value rising by 0.0115 from 0.0874 to 0.0989.

\indent Notably, cold wave shocks generate a more significant impact than heat wave shocks. The demand response values at 3.46°C, 1.06°C, and -1.53°C are 0.2138, 0.2794, and 0.2806, respectively. These empirical results indicate that when the average temperature decreases from 3.46°C to 1.06°C during a moderate cold wave, the year-over-year monthly demand growth rate is 6.56\% higher than the year-over-year monthly growth rate observed at 3.46°C. Additionally, as the temperature drops further from 1.06°C to -1.53°C during an extreme cold wave, the year-over-year monthly demand growth rate increases by an additional 0.12\% compared to the year-over-year monthly growth rate at 1.06°C. It is important to note that the FSR model with $\kappa=0$, which does not account for measurement error, fails to identify such nonlinearity. Moreover, utilizing Legendre basis functions results in a slightly lower temperature sensitivity in magnitude, but the overall shape of the sensitivity curve remains nearly identical to that obtained using Fourier basis functions.

\indent The observation that cold wave shocks significantly increase electricity demand more than heat wave shocks implies that electricity demand is more sensitive to the more intense and extreme temperature conditions associated with cold waves. This further implies that the demand response is not just a function of temperature extremes but also the nature of these extremes. This finding departs from existing literature, which primarily focuses on the demand response to temperature level changes alone, and highlights the importance of understanding how shifts in temperature distributions impact electricity demand. Such insights emphasize the need for energy planning that accounts for the varying effects of temperature distribution changes, particularly in the context of increasingly severe cold wave events.

\indent The existing functional approach is susceptible to boundary issues, particularly in estimating the nonlinear relationship between temperature and electricity demand using a functional Fourier flexible form (\citealp{gallant1981bias}; \citealp{chang2016new}). A notable drawback of this method is its tendency to produce inaccurate estimates at the boundaries, especially in regions where data are sparse, such as around the critical temperature thresholds of -20°C and 40°C. These boundary estimates are economically significant, as they can lead to substantial implications in policy and energy management. In contrast, our approach does not focus on the demand response at specific temperature levels but rather generates hypothetical functional shocks to analyze the impact of extreme temperatures. This approach is less prone to boundary issues, providing more reliable estimates by effectively circumventing the problems associated with critical temperature points.

\indent Note that our approach involves addressing the measurement error problem to mitigate potential endogeneity issues. If endogeneity exists, it can bias the nonlinear response estimates. The IV approach corrects this bias by using instruments that are correlated with the endogenous regressors but uncorrelated with the error term. However, this correction may introduce larger standard errors and increased variance, which can diminish the model's goodness of fit—meaning the model may not align as closely with the observed data compared to the standard functional approach. This trade-off becomes apparent in our results with orthonormal Fourier (Legendre) Basis functions, as reflected by the Root Mean Squared Error (RMSE) values are recorded as 0.0822 (0.0822) and 0.1227 (0.1222) for $\kappa = 0$ and $1$, respectively.

\bigskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Empirical Results for Quantile-to-Demand Model} 
\noindent Some might wonder if the quantile function models \commWK{capture} extreme temperature events more effectively than the density function. Specifically, the difference lies in how each approach handles the heterogeneous impact of temperature on electricity demand. The temperature density-to-demand model accounts for the varying influence of each temperature level on demand, whereas the temperature quantile-to-demand model considers the heterogeneous effects of temperature quantiles on demand. As a result, while the density function may more accurately capture the average fluctuations in electricity demand, the quantile function, despite its relatively lower model fit, may be better suited to explaining demand responses under extreme temperature conditions. For instance, during a heat wave, where consumers face unprecedented temperatures, the relevance of past temperature impacts (as modeled by the density function) may diminish, making the quantile function more effective in modeling demand changes at extreme temperatures. In addition, the quantile function would better manage the heterogeneous support of the temperature density function.

%\indent Note that the cumulative temperature effect refers to the phenomenon where prolonged periods of high or low temperatures lead to an increased demand for cooling or heating, respectively, even when the actual temperature level remains constant. This seemingly paradoxical rise in electricity demand occurs because sustained exposure to extreme temperatures exacerbates the need for maintaining indoor climate conditions. Given that quantile functions directly capture how extreme temperature values accumulate across different quantiles, they could be effective in assessing the impact of prolonged high temperatures on electricity demand. By focusing on the tails of the distribution, quantile functions may highlight the increased demand that arises from upper- or lower-end temperature quantiles.

\indent In this context, we further examine the effects of temperature quantiles on electricity demand for extreme weather events. The left panel of Figure \ref{Fig:Quantile_Descrip} displays the \commWK{temporal mean, standard deviation, skewness, and kurtosis at various qunatile levels (which are computed from the time series $\{X_t(u)\}_{t=1}^T$ for each $u \in [0,1]$}), providing insights into how the temperature changes across different quantiles. The mean temperature increases steadily across the quantiles, reflecting the expected rise in temperature values from lower to higher quantiles. The standard deviation decreases, indicating that temperature values become less variable at higher quantiles. The skewness becomes more negative as the quantile increases, signifying that higher temperatures are more concentrated towards their upper range, leading to a more skewed distribution. Conversely, kurtosis decreases initially but sharply increases at the highest quantiles, suggesting a less peaked distribution initially but with more pronounced tails, indicating more frequent extreme temperature events in these higher quantiles. The right panel of Figure \ref{Fig:Quantile_Descrip} shows kernel density estimates for the 1st to 4th \commWK{quartiles}. The density curves illustrate that lower \commWK{quartiles} (1st and 2nd) are more tightly clustered, while higher \commWK{quartiles} (3rd and 4th) exhibit greater dispersion, reflecting the variability and occurrence of extreme temperatures in these ranges. 

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.4\textwidth, width=0.48\textwidth]{FRKETQ_P3/Quant_desc1.png}
\includegraphics[height=0.4\textwidth, width=0.48\textwidth]{FRKETQ_P3/Quant_desc2.png}
\caption{Descriptive statistics of quantile function for each temperature quantile (left) and kernel density estimates of four quantile ranges (right).}
\label{Fig:Quantile_Descrip}
\end{center}
\end{figure}

\indent Note that the statistical relationship between the temperature quantile function and electricity demand varies seasonally. During summer, the positive relationship is observed as higher temperatures increase cooling demand, while in winter, the negative relationship is observed due to the increased heating demand at lower temperatures. As it turns out that the negative effects during winter outweigh the positive effects in summer, the overall effect of the quantile function at each temperature quantile on electricity demand becomes negative. As illustrated in Figure \ref{Fig:Quantile_Descrip}, moreover, the temperature quantile function at the high quantile exhibits lower volatility and skewness but significantly higher kurtosis compared to that at the low quantile. This distinction indicates that while temperature fluctuations are less pronounced at higher quantiles, extreme values (peaks) occur more frequently, leading to a sharper distribution. As a result, the effects of the temperature quantile function at the low quantile on electricity demand are notably smaller than those at the high quantile. This finding highlights a unique characteristic of the quantile function, as it can capture relationships that density functions cannot, given that density functions are constrained to non-negative values. 

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.3\textwidth, width=0.99\textwidth]{FRKETQ_P3/Quant_Shock.png}
\includegraphics[height=0.3\textwidth, width=0.99\textwidth]{FRKETQ_P3/Quantile_shock_Desc.png}
\caption{Estimated quantile functions and functional shocks for cold wave (top left) and heat wave (top right). The functional quantile shocks for cold (blue) and heat (red) waves are shifted for modest cold wave (blue dotted) and heat wave shocks (red dotted) in the bottom left panel. The mean change of the upper (line) and lower (dotted) tenth quantiles of the functional quantile shocks during the shifting process (bottom right).}
\label{Fig:Quantile_Shock}
\end{center}
\end{figure}

\indent The top left panel of Figure \ref{Fig:Quantile_Shock} illustrates the quantile shocks for the cold wave, where the impact is most pronounced in the lower quantiles, especially those associated with the coldest temperatures. This reflects that the January 2021 cold wave caused a significant downward shift in the quantile function compared to January 2020, with the most substantial changes at the lowest quantiles. On the top right panel, the quantile shocks for the heat wave reveal a more uniform increase across the quantiles, with a greater effect at the higher quantiles. This suggests that the August 2018 heat wave led to a consistent rise in temperatures, primarily intensifying extreme high-temperature events. 

\indent The bottom two panels in Figure \ref{Fig:Quantile_Shock} illustrate the functional quantile shocks for both cold wave and heat wave events as a result of shifting the quantile functions in Figure \ref{Fig:Func_shock3}.\footnote{The sequence of quantile shocks with varying cold and heat wave intensities is generated by adding the density function in January 2020 and August 2017 to the sequence of temperature density shocks in the left panel of Figure \ref{Fig:Func_shock3}. This addition is followed by transforming the resulting density functions into their respective quantile functions.} More specifically, the bottom left panel shows the dotted blue (red) line representing quantile shocks generated by modest cold (heat) waves, while the solid blue (red) line reflects the strongest cold (heat) wave shocks. These shocks arise from the temperature quantile shifts under varying cold or heat wave intensities. In the bottom right panel, moreover, the solid (dotted) red line illustrates the mean changes of the upper (lower) tenth quantiles for heat wave shocks during the shifting process, while the solid (dotted) blue line indicates the same for cold wave shocks. Note that we include an additional Fourier or Legendre basis function corresponding to the constant term because the upward or downward quantile shifting shocks generate a mean change. Unlike the density-to-demand model with CLR transformation, restricting the constant term of the basis function to zero would result in identical quantile shocks across the temperature quantiles.

%\indent While density and quantile functions exhibit similar mean, these two functions differ significantly due to the distinct ways each function encapsulates data characteristics. Density functions directly reflect the probability distribution, effectively capturing the central tendency, spread, asymmetry, and tail behavior. In particular, skewness reveals the asymmetry of a distribution, while kurtosis measures tail thickness and central peak sharpness, providing key insights into distribution shape and tail behavior. On the other hand, quantile functions excel at describing extreme values, capturing the temperature's change at the tails more effectively than skewness and kurtosis alone. These statistical differences indicate that critical information, such as skewness and kurtosis of the temperature density function, would be missed when relying solely on quantile functions in electricity demand modeling. Thus, combining both functions enhances explanatory power, particularly for modeling extreme temperatures or other tail-heavy phenomena. 

%In contrast, quantile functions, being more responsive to extreme values across the distribution, can show disparities in skewness and kurtosis even when the mean and variance are aligned. Specifically, the sample correlations between the time series of temperature density and quantile functions for mean, variance, skewness, and kurtosis are 1, 0.71, -0.36, and 0.01, respectively. 

%\indent In this context, we consider augmenting the quantile-to-demand model with demeaned skewness and kurtosis of the temperature density function to improve the precision of demand response estimation. One caveat is, however, that this augmentation assumes that the heat wave and cold wave shocks generated by the quantile functions do not alter the skewness and kurtosis of the temperature density function. This presumption may overlook the potential impact that is induced by changing these higher-order moments. 

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.3\textwidth, width=0.35\textwidth]{FRKETQ_P3/Quant_Sensitivity.png}
\includegraphics[height=0.3\textwidth, width=0.6\textwidth]{FRKETQ_P3/Quant_Est_rlt.png}
\caption{Estimated temperature quantile sensitivity (left) and quantile-based temperature sensitivity for varying cold wave (top right) and heat wave (bottom right) shock intensities under $\kappa = 0$ and $\kappa = 1$, using Fourier (blue and red) and Legendre (black) basis functions. The dotted lines indicate the 95\% local confidence intervals with the Fourier basis function.}
\label{Fig:Quantile_non_est}
\end{center}
\end{figure}
% 

\indent The left panel of Figure \ref{Fig:Quantile_non_est} provides the temperature quantile sensitivity with respect to the residential electricity demand. To approximate $\hat{f}$ in equation \eqref{eqest} in the local context and interpret its impact on electricity demand, we start by constructing \( x \) as a sequence of indicators. This approach enables us to focus on approximating $\hat{f}$, allowing for a more refined resolution in approximating $\hat{f}$ values as permitted by the data. Once an accurate local approximation of $\hat{f}$ is obtained, we can examine $\hat{f}(x)$, the value of $\hat{f}$ at a specific \( x \). Specifically, $\hat{f}(x)$ represents the effect of a change in a given quantile while other quantiles remain fixed, akin to the interpretation in linear regression. However, in reality, it is rare for a single quantile to shift independently of others, which can introduce interpretational ambiguities despite the robustness of the approximation.

\indent To address this, we introduce a concept of total quantile change, denoted as \( Q \), to capture the cumulative impact of quantile adjustments. Starting with an even shock from the \( 0.5 \) quantile to the \( 1 \) quantile, \( Q \) is distributed uniformly over this range, represented as a step function with a value of \( 1 \) from \( x = 0.5 \) onward, where \( Q = 0.5 \times 1 = 0.5 \). Subsequently, we increase the quantile range incrementally (e.g., from the \( 0.55 \) quantile to the \( 1 \) quantile) while maintaining the same \( Q \), thus gradually concentrating the quantile change at higher quantiles. Conversely, for a negative shock of \( -Q \), we consider evenly reducing quantiles from the lower end, concentrating the change in lower quantiles. By analyzing the function $\hat{f}(x)$ across these step function sequences, we can observe how electricity demand responds to quantile shocks concentrated at various parts of the distribution, providing insights into which quantile ranges most significantly influence demand. 

\indent Not surprisingly, the estimated temperature quantile sensitivity exhibits a U-shaped pattern, consistent with findings from \cite{chang2014time} regarding temperature density sensitivity. However, unlike \cite{chang2014time}, the nonlinearity in cooling demand was found to be statistically insignificant. In contrast, the heating demand demonstrates statistically significant sensitivity to temperature changes. Notably, when the temperature rises above the 0.4 quantile, electricity demand decreases, with this reduction intensifying up to the 0.7 quantile before gradually diminishing. This behavior reveals a unique nonlinear pattern in the relationship between temperature quantile and electricity demand, highlighting the asymmetrical effects of temperature on electricity demand across different quantiles.

\indent The right panel of Figure \ref{Fig:Quantile_non_est} presents the estimation results of extreme temperature events from the Fourier- and Legendre-based quantile-to-demand model with 95\% local confidence intervals. Unlike the density-to-demand approach, the quantile-based model fails to capture nonlinear temperature sensitivity with statistical significance. The absence of nonlinearity may be due to the quantile-to-demand model's limitations in explaining the time series pattern of electricity demand using the cumulative temperature effects. The RMSE values from the quantile-to-demand model are 0.0933 (0.0933) and 0.1375 (0.1456) when using orthonormal Fourier (Legendre) basis function for $\kappa = 0$ and $1$, respectively. These results indicate a decline in the goodness of fit compared to the density-to-demand model.

%Figure \ref{Fig:Quantile_non_est} clearly demonstrates the necessity of incorporating higher-order moments of temperature density function into the quantile-to-demand model. Ignoring these moments consistently results in underestimating demand response, whether assuming no measurement error or serially uncorrelated error. However, it turns out that the quantile-to-demand model no longer shows increasing temperature sensitivity. Unlike the density-to-demand approach, the quantile-based model fails to capture nonlinear temperature sensitivity. This absence of pronounced changes may be due to the quantile-to-demand model’s inability to fully account for higher-order temperature effects, which are crucial for reflecting demand response under extreme conditions. As a result, the quantile-based model may oversimplify the relationship between temperature variations and electricity demand, leading to the observed flat response. %Notably, the quantile-based approach exhibits more pronounced sensitivity to extreme temperature conditions compared to the density-based results, with significant increases in electricity demand under extreme cold and heat waves when higher-order moments are considered and $\kappa=1$ is applied. This comparison highlights the superior ability of the quantile-based approach to capture demand responses under extreme temperature conditions.%, underscoring the critical role of accounting for non-linear characteristics in temperature distributions.






==> FRKETQ_P3/05_FRKET_Conclude.tex <==
\noindent In this paper, we estimate the nonlinear temperature sensitivity of residential electricity demand while accounting for measurement errors. Given that residential electricity demand is highly sensitive to temperature fluctuations, accurately capturing these nonlinearities is critical, especially during extreme temperature events where underestimation could jeopardize grid stability. Additionally, measurement errors often stem from the assumption that nonparametrically estimated temperature densities represent true densities, compounded by data quality issues and limitations within the estimation process.

\indent We tackle these challenges by applying a function-to-scalar regression to both temperature density-to-demand and quantile-to-demand models. This approach enables us to effectively identify nonlinearities in the relationship between temperature distribution and electricity demand, even when measurement errors are present. Through the analysis of historical heat wave and cold wave shocks of varying intensities within a distributional context, we discover that residential electricity demand is significantly more sensitive to the extreme conditions associated with intense cold waves. Additionally, the temperature quantile-to-demand model fails to yield reliable estimates.

\indent Given our findings, energy practitioners should prioritize incorporating detailed temperature distribution analysis, particularly when planning for extreme weather events. Our empirical results reveal that residential electricity demand is more sensitive to intense cold waves than to heat waves, highlighting the need for robust demand forecasting models that account for these nonlinear sensitivities. Moreover, it is crucial to address potential measurement errors by adopting advanced techniques, in order to ensure that demand response strategies are based on accurate and reliable estimates. Our econometric approach would enhance grid stability and support effective energy management during extreme temperature events.









